The Multiscale Bowler-Hat Transform for Vessel Enhancement in 3D Biomedical Images

Enhancement and detection of 3D vessel-like structures has long been an open problem as most existing image processing methods fail in many aspects, including a lack of uniform enhancement between vessels of different radii and a lack of enhancement at the junctions. Here, we propose a method based on mathematical morphology to enhance 3D vessel-like structures in biomedical images. The proposed method, 3D bowler-hat transform, combines sphere and line structuring elements to enhance vessel-like structures. The proposed method is validated on synthetic and real data and compared with state-of-the-art methods. Our results show that the proposed method achieves a high-quality vessel-like structures enhancement in both synthetic and real biomedical images, and is able to cope with variations in vessels thickness throughout vascular networks while remaining robust at junctions.

==> tex/document.tex <==



==> tex/figure-real-data.tex <==
\renewcommand\hfigure{1}
\renewcommand\wfigure{1}
\renewcommand\bfigure{0.25}
\begin{figure}
	\centering
	\begin{subfigure}[t]{\bfigure\linewidth}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] (image) at (0,0) 
		{\includegraphics[trim={0px 0px 0px 30px}, clip,width=\wfigure\linewidth,keepaspectratio=true]{MAP4.png}};
		\begin{scope}[x={(image.south east)},y={(image.north west)}]
		\draw[red,thick,] (0.8,0.9) rectangle (0.5,0.6);
		\end{scope}
		\end{tikzpicture}
		\caption{\quad}\label{fig:OrCel}
	\end{subfigure}
	\begin{subfigure}[t]{\bfigure\linewidth}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] (image) at (0,0) 
		{\includegraphics[width=\wfigure\linewidth,keepaspectratio=true]{keratin2}};
		\begin{scope}[x={(image.south east)},y={(image.north west)}]
		\draw[red,thick,] (0.48,0.3) rectangle (0.83,0.67);
		\end{scope}
		\end{tikzpicture}
		\caption{\quad}\label{fig:OrKer}	
	\end{subfigure}
	\begin{subfigure}[t]{\bfigure\linewidth}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] (image) at (0,0) 
		{\includegraphics[trim={10px 100px 10px 0px}, clip, width=\wfigure\linewidth, keepaspectratio=true]{LuciferS.png}};
		\begin{scope}[x={(image.south east)},y={(image.north west)}]
		\draw[red,thick,] (0.2,0.38) rectangle (0.8,0.95);
		\end{scope}
		\end{tikzpicture}
		\caption{\quad}\label{fig:OrNeurite}
	\end{subfigure}
\vspace{-10px}
	\caption{2D max projections of 3D images of microtubules network in plant cell (\subref{fig:OrCel}) and keratin network in skin cell (\subref{fig:OrKer}) (provided by Dr Tim Hawkins, Durham University, UK),  and neuronal network (\subref{fig:OrNeurite}) (provided by Dr Chris Banna, UC Santa Barbara, USA). Regions of interest are highlighted in red.}	\label{fig:original}\vspace{-10pt}	
\end{figure}

==> tex/figure-spiral.tex <==
% !TEX root = ../icpr.tex
\begin{figure}
	\centering
	\begin{subfigure}[t]{0.5\linewidth}
		\centering
		\includegraphics[width=\linewidth,keepaspectratio=true]{spiral}
		\end{subfigure}
	\caption{Uniform distribution of 700 points over the surface of a sphere \cite{saff1997distributing}. }\label{fig:spiral}\vskip-15pt
\end{figure}

==> tex/figure-vascusyn-illum.tex <==
\renewcommand\bfigure{0.15}
\begin{figure}[b!]
	\centering
	\begin{subfigure}[t]{\bfigure\linewidth}
		\centering
		\includegraphics[width=\linewidth,keepaspectratio=true]{no}
		\caption{Original}\label{fig:shadow}
	\end{subfigure}
	\begin{subfigure}[t]{\bfigure\linewidth}
		\centering
		\includegraphics[width=\linewidth,keepaspectratio=true]{no}
		\caption{Level 10}\label{fig:shadow10}
	\end{subfigure}
	\begin{subfigure}[t]{\bfigure\linewidth}
		\centering
		\includegraphics[width=\linewidth,keepaspectratio=true]{no}
		\caption{Level 50}\label{fig:shadow50}
	\end{subfigure}
	\begin{subfigure}[t]{\bfigure\linewidth}
		\centering
		\includegraphics[width=\linewidth,keepaspectratio=true]{no}
		\caption{Level 100}\label{fig:shadow100}
	\end{subfigure}
	\begin{subfigure}[t]{\bfigure\linewidth}
		\centering
		\includegraphics[width=\linewidth,keepaspectratio=true]{no}
		\caption{Level 150}\label{fig:shadow150}
	\end{subfigure}
	\begin{subfigure}[t]{\bfigure\linewidth}
		\centering
		\includegraphics[width=\linewidth,keepaspectratio=true]{no}
		\caption{Level 200}\label{fig:shadow200}
	\end{subfigure}
	\caption{Example of generated volumes using VascuSynth in different level of shadow affect has been tested by proposed method. (\subref{fig:shadow})~is the original vasculature structures with the maximum intensity projections. (\subref{fig:shadow10}-\subref{fig:shadow200})~demonstrate the proposed method results on the variety of shadow affects.}
\end{figure}

==> tex/implementation.tex <==
\section{Implementation}
%\subsection{Runtime}
\label{sec:implementation}
All codes were implemented and written in MATLAB 2015a on Windows 8.1 pro 64-bit PC running an Intel Core i7-4790 CPU (3.60 GHz) with 16GB RAM.

==> tex/introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%INTRODUCTION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-20px}
\section{Introduction}
\label{sec:intro}
\vspace{-10px}
 Enhancement of curvilinear structures is an important preprocessing step for the further image analysis methods like segmentation or registration. Consequently, a robust and durable image enhancement of curve-like features is a general requirement for bioimage processing. Several image enhancement methods have been proposed in the literature such as;  blood vessels~\cite{Benmansour2011,frangi1998multiscale}, neurones~\cite{al2008improved}, microtubules~\cite{hadjidemetriou2005segmentation} and others~\cite{lesage2009review}.
 Nevertheless, most of the methods have problems, losing signals at the junctions, false vessel affects or exposed vessels too much.
 The paper is organised as follows: discussion of the most common image processing methods for intensity and phase-based enhancement of curvilinear structures is presented in Section \ref{sec:related}. In Section \ref{sec:proposed:method}, we formulate the 3D bowler hat transform. Experimental results for 3D synthetic and real biological images are presented in Section \ref{sec:results}. Section \ref{sec:conclusion} is dedicated to conclusions discussion.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%RELATED WORK
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-10px}
\section{Related Work}
\label{sec:related}
\vspace{-5px}
\subsection{Hessian-based Enhancement Methods}
\label{subsec:hessian}
At the first place, Frangi and his colleagues~\cite{frangi1998multiscale} enhanced the curvilinear structures in 2/3D by using the eigenvalues of Hessian matrices, and most of the methods related to image enhancement originated from their work as seen in~\cite{frangi1998multiscale,krissian2000model}. Hessian matrix can be defined in 3D as:
\begin{align}
	H=\begin{bmatrix} H_{ 11 } & H_{ 12 } & H_{ 13 } \\
	H_{ 21 } & H_{ 22 } & H_{ 23 } \\
	H_{ 31 } & H_{ 32 } & H_{ 33 } 
	\end{bmatrix}=
	\begin{bmatrix} \displaystyle \frac{\partial^2I}{\partial x^2}*G_\sigma & 
	\displaystyle \frac{\partial^2I}{\partial x\partial y }*G_\sigma &
	\displaystyle \frac{\partial^2I}{\partial x\partial z }*G_\sigma \\
	\displaystyle \frac{\partial^2I}{\partial x\partial y }*G_\sigma& 
	\displaystyle \frac{\partial^2I}{\partial y^2 }*G_\sigma & 
	\displaystyle \frac{\partial^2I}{\partial y\partial z }*G_\sigma \\
	\displaystyle \frac{\partial^2I}{\partial x\partial z }*G_\sigma &
	\displaystyle \frac{\partial^2I}{\partial y\partial z }*G_\sigma &
	\displaystyle \frac{\partial^2I}{\partial z^2 }*G_\sigma
	\end{bmatrix}.
\end{align}
$H$ is symmetric and positive semi-definite that has two orthogonal eigenvectors and eigenvalues as follows;
\begin{align}
\label{eq:lambdaCalculation}
& \lambda_{ 1,2 }=\frac { 1 }{ 2 } \left( { H }_{ 11 }+{ H }_{ 22 } \pm\sqrt { \left( { H }_{ 11 }-{ H }_{ 22 } \right) ^{ 2 }+4{ H }_{ 12 }^{ 2 } }  \right).
\end{align}
We characterize Hessian-based enhancement methods in respectively; vesselness as in~\cite{frangi1998multiscale}, neuriteness as described in~\cite{meijering2004design} and a recently proposed measurement based on the regularised volume ratio in~\cite{JPLetal2016}.
\vspace{-15px}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%VESSELNESS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Vesselness}
\label{subsec:ves}
Vesselness~\cite{frangi1998multiscale} is calculated by computing the ratio of eigenvalues of Hessian matrix $H_s(\mathbf{p})$:
\begin{equation}
\label{eq:Vesselness}
\resizebox{.9\hsize}{!}{$
	V_s = \begin{cases}
	0 & \quad \lambda_{s,2}, \lambda_{s,3}<0 \\
	\text{exp}\left({-\dfrac{R_{\beta}^2}{2\beta^2}}\right)
	\Bigg(1-\text{exp}\left({-\dfrac{R_\alpha^2}{2\alpha^2}}\right)\Bigg) 
	\Bigg(1-\text{exp}\left({-\dfrac{S^2}{2c^2}}\right)\Bigg) & \quad \text{otherwise}
	\end{cases},$}
\end{equation}
where
\begin{equation}
	S = \sqrt{ \lambda_{s,1}^{2} + \lambda_{s,2}^{2} + \lambda_{s,3}^{2} }
	,\quad
	R_{\beta} = \frac{{\left|\lambda_{s,1}\right|}}{\sqrt{\left|\lambda_{s,2}\lambda_{s,3}\right|}}
	,\quad	
	R_{\alpha} = \frac{\left|\lambda_{s,2}\right|}{\left|\lambda_{s,3}\right|},
\end{equation}	
where  $\alpha $, $\beta$  and $c$  are positive real user-defined parameters. The $R_\beta$ ratio determines blob-like features~\cite{frangi1998multiscale} and the $R_\alpha$ ratio helps to distinguish between plate-like and line-like structures~\cite{jerman2015beyond}. $S$ is equal to half of the maximum Frobenius norm~\cite{antiga2007generalizing}
and evaluates whether the eigenvalues are large compared to noise. Several structure models have been found to express the eigenvalues of Hessian matrix~\cite{krissian2000model}, see Table~\ref{table:Hessian3d}.
Finally, multi-scale vesselness, for a given set of scales ${\sum=\{s_i\}} $ and $i={1,2,3...}$, 
can be calculated as~\cite{obara2012contrast}:
\begin{equation}
	V_{\sum} = \underset{s \in \sum} \max \left( V_s \right).
\end{equation}
\begin{table}[b!]
	\centering
	\captionsetup{font=normal}
	\caption{Possible patterns in 3D, depending on the eigenvalues of Hessian matrix (L low, H+ high positive, H- high low)}\label{table:Hessian3d}
	\resizebox{.35\linewidth}{!}{
		\begin{tabular}{@{}lllll@{}}
			\toprule
			\multicolumn{4}{c}{\textbf{3D}}\\ \midrule \hline
			$\lambda_1$ & $\lambda_2$ & $\lambda_3$& \textbf{Structure}\\ \midrule
			L  & L  & L  & Background       \\ 
			L  & L  & H- & Bright sheet		\\ 
			L  & L  & H+ & Dark sheet  		\\ 
			L  & H- & H- & Bright tubular   \\ 
			L  & H+ & H+ & Dark tubular     \\ 
			H- & H- & H- & Bright blob  	\\ 
			H+ & H+ & H+ & Dark blob    	\\ \bottomrule
	\end{tabular}}
\end{table}
Vesselness fails at junctions without any kind of tracking methods because eigenvalues become zero at junctions.
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%NEURITENESS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Neuriteness}
\label{subsec:neurite}
Neuriteness is another implementation of the vessel detection based on Hessian matrix. Firstly, it has been proposed by \cite{meijering2004design} for the 2D case then it is extended to 3D in~\cite{al2008improved}. It is required second-order derivatives of the Gaussian Kernel with a given scale $s$. The Neuriteness method consists of a detection stage~\cite{levitan2015neuron}, that implies a feasible neurite in the every individual pixel in the image, has a non-zero value; and actual tracing stage~\cite{capowski1989computer}, determines the pixels which should be neurites, most likely to reflect the center-lines of neurites. Neuriteness using the sort of modified Hessian matrix by adding the parameter $\alpha$.  For the 3D case modified Hessian matrix ${ H }^{ ' }$ is: 
	\begin{equation} 
	\label{eq:neuriteness}
	{ H }^{ ' } =\begin{bmatrix} { H }_{ 11 }  +\frac { \alpha  }{ 2 } { H }_{ 22 }  +\frac { \alpha  }{ 2 } { H }_{ 33 }   & \left( 1-\alpha  \right) { H }_{ 12 }   & \left( 1-\alpha  \right) { H }_{ 13 }   \\ \left( 1-\alpha  \right) { H }_{ 12 }   & { H }_{ 22 }  +\frac { \alpha  }{ 2 } { H }_{ 11 }  +\frac { \alpha  }{ 2 } { H }_{ 33 }   & \left( 1-\alpha  \right) { H }_{ 23 }   \\ \left( 1-\alpha  \right) { H }_{ 13 }   & \left( 1-\alpha  \right) { H }_{ 23 }   & { H }_{ 33 }  +\frac { \alpha  }{ 2 } { H }_{ 11 }  +\frac { \alpha  }{ 2 } { H }_{ 22 }   \end{bmatrix}.
	\end{equation}
The parameter $\alpha$ is proposed optimal value by \cite{meijering2004design}. 3D neuritenees measurement can defined as:
\begin{equation}
\label{eq:Neuriteness}
N=
\begin{cases}
	\dfrac{\lambda_{\max}}{\lambda_{\min}} \quad & $if$\quad \lambda_{\max} <0,\\
	0\quad &  $if$\quad \lambda_{\max}\ge 0,
\end{cases}
\end{equation}
where
\begin{align}
	&\lambda_1^{'} =\lambda _ 1 +\alpha \lambda _{ 2 }+\alpha \lambda _{ 3 },\\
	&\lambda_2^{'}=\lambda _{ 2 } +\alpha \lambda _{ 1 }+\alpha \lambda _{ 3 },\\
	&\lambda_3^{'}=\lambda _{ 3 } +\alpha \lambda _{ 1 }+\alpha \lambda _{ 2 },\\
	&\lambda_{\max} =\max(|{\lambda_{1}}'|,|{\lambda_{2}}'|,|{\lambda_{3}}'|),\\
	&\lambda_{\min} =  \min(\lambda_{\max}),
\end{align}
where  $ { \lambda  }_{ i }^{ ' }$ are the normalized eigenvalues of $H'$; $\lambda_{\max}$ is the largest eigenvalue at each pixel; and $\lambda_{\min}$ the smallest of all $\lambda_{\max}$~\cite{meijering2004design}. Neuriteness also inherits junction problem from eigenvalues of Hessian matrix.
\vspace{-5px}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%REGULARIZED VOLUME RATIO
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Regularized Volume Ratio}
\label{subsec:volrat}
A problem with the Hessian approaches such as the vesselness measure is the direct proportionality of the enhancer on $\lambda_{2,3}$ and due to eigenvalue heterogeneity within objects and variation in eigenvalue magnitude this proportionality results in non-uniform enhancement. In~\cite{JPLetal2016} attempt to solve this problem by deriving a modification of the volume ratio with a regularised $\lambda_3$ to ensure robustness to small changes in magnitude, \textit{e.g.} noise. Their solution is given by
\begin{equation}
	\mathcal{V}_P=
	\begin{cases}
		0                                                                               & \text{if}~\lambda_2 \le 0 \lor \lambda_{\rho} \le 0, \\
		1                                                                               & \text{if}~\lambda_2 \ge \lambda_{\rho}/2 > 0,        \\
		\lambda_2^2(\lambda_{\rho} - \lambda_2)[\frac{3}{\lambda_2 + \lambda_{\rho}}]^3 & \text{otherwise},
	\end{cases}
\end{equation}
where $\lambda_{\rho}$ is the regularised form of $\lambda_3$, given by
\begin{equation}
	\lambda_{\rho}(s) =
	\begin{cases}
		\lambda_3                                  & \text{if}~\lambda_3 > \tau\max_\mathbf{p}\lambda_3(\mathbf{p},s),       \\
		\tau\max_\mathbf{p}\lambda_3(\mathbf{p},s) & \text{if}~0 < \lambda_3 \le \tau\max_\mathbf{p}\lambda_3(\mathbf{p},s), \\
		0                                          & \text{otherwise},
	\end{cases}
\end{equation}
for scale $s$, where $\tau$ is a cut-off threshold between zero and one.
\vspace{-5px}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%PHASE CONGRUENCY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Phase Congruency-based Enhancement Methods}
\label{subsec:pc}
Most image enhancement methods have a common problem of image contrast and spatial magnification dependency, which causes fine, lower contrast vessels to be missed~\cite{kovesi1996invariant}.
To overcome this problem, contrast-independent image enhancement measurement, namely phase congruency, has been proposed in~\cite{obara2012contrast} and extended to 3D by~\cite{sazak2017contrast}. 
The phase congruency detects features as the points where Fourier phase components align~\cite{morrone1986mach}.
Since the concept of local phase is naturally a 1D function,there is no direct extension for 2/3D versions and also the original measurement is not robust against the noise; then Kovesi et al.~\cite{kovesi2003phase,kovesi2000phase,kovesi1999image,kovesi1996invariant} have proposed 2/3D  phase congruency approach that combines both sine and cosines phase elements, improving the localisation information and noise robustness.
\subsubsection{3D Phase-based Enhancement}
\label{subsec:3DPhaseBasedEnhancement}
The local phase is required a variety of orientations in order to obtain complete phase congruency in 2/3D as shown by~\cite{kovesi1999image}. As mentioned in above section, there is no straightforward implementation of 2/3D phase congruency because of the nature of local phase function. Consequently, quadrature pairs are required to calculate in 2/3D. 
 Accordingly, for a given image $I({\mathbf{p}})$ and a quadrature pair of even $F_{s,\Theta}^{e}$ and odd $F_{s,\Theta}^{o}$ filters at scale $s$ and orientation $\Theta$, the response vector is given by its even and odd components $e_{s,\Theta}(\mathbf{p})$ and $o_{s,\Theta}(\mathbf{p})$:
\begin{equation}
\left[ e_{s,\Theta}\left(\mathbf{p}\right), o_{s,\Theta}\left(\mathbf{p}\right) \right] 
= \left[ I\left(\mathbf{p}\right) \ast F_{s,\Theta}^{e}, I\left(\mathbf{p}\right) \ast F_{s,\Theta}^{o} \right].
\end{equation}
The amplitude of the $s^{th}$ component $A_{s,\Theta}\left({\mathbf{p}}\right) $ is defined as:
\begin{equation}
A_{s,\Theta}\left({\mathbf{p}}\right) = 
\sqrt{e_{s,\Theta}\left(\mathbf{p}\right)^2 + o_{s,\Theta}\left(\mathbf{p}\right)^2 },\quad 
\varphi_{s,\Theta}\left({\mathbf{p}} \right) = 
atan\left(\frac{o_{s,\Theta}\left(\mathbf{p}\right) }{ e_{s,\Theta}\left(\mathbf{p}\right)} \right),
\end{equation}
where $\varphi_{s,\Theta}\left({\mathbf{p}} \right)$ is the local phase. Since the Fourier transform is computationally expensive, the Log-Gabor filter has been used to estimate local phase of phase congruency.
The several orientation quadrature filters calculated by 3D Log-Gabor filter~\cite{Wang2008301}. It has two components of the Gaussian transfer function on the logarithmic frequency domain~\cite{Wang2008301}. 
In the light of these information, the 3D phase congruency  is computed as the sum of phase congruencies at several orientations~\cite{ferrari2011detection}:
\begin{equation}
\text{PC}(\mathbf{p}) = \sum_{\Theta}\left(\text{PC}_{\Theta}(\mathbf{p})\right),
\end{equation}
and the phase congruency at each orientation $\Theta$ is defined as:
\begin{equation}
\text{PC}_{\Theta}(\mathbf{p}) = 
\frac {{\sum}_{s}w_{\Theta}(\mathbf{p})\max (A_{s,\Theta}(\mathbf{p})\Delta\Phi_{s,\Theta}(\mathbf{p})-t,0)}
{{\sum}_{ s }A_{s,\Theta}(\mathbf{p})+\varepsilon}.
\label{eq:pahse1}
\end{equation}
$A_{s,\Theta}(\mathbf{p})$ is the amplitude of the image component at the location $\mathbf{p}$. The $t$ is a noise threshold and $\varepsilon$ a factor that ensures against the division of zero~\cite{kovesi1999image}. $w_\Theta(\mathbf{p})$ is the weight of frequency spread which penalizes frequency distributions. Lastly, $\Delta\Phi_{s,\Theta}(\mathbf{p})$ is a phase deviation. More details in ~\cite{sazak2017contrast}.
\vspace{-5px}
\subsubsection{3D Tensor Based Phase Congruency with Vesselness and Neuriteness} 
\label{sec:PCTNeVes}
Combining a polar separable quadrature filters across the dominant orientation, it is possible to get how features differentiate along the image. One of the common strategy is to represent the local structure with the tensor. Within the neighbourhood of $\textbf{p}$, the appropriate notation is given by the tensor as follows:
\begin{equation}
T=\sum_{\Theta}\|q_{\Theta}\|(\mathbf{u}_{\Theta}\mathbf{u}_{\Theta}^T),
\label{eq:tensor}
\end{equation}
where $q_{\Theta}$ is the output of oriented quadrature filter in the direction specified by $\Theta$, and $\mathbf{u}_{\Theta}$ is the column vector:
\begin{equation}
\mathbf{u}_\Theta=\mathbf{u}_{\theta,\phi} = [sin(\theta)cos(\phi), sin(\theta)sin(\phi), cos(\theta)]^T.
\end{equation} 
Analysing the relationship between eigenvalues and eigenvectors of Hessian allow us to enhance curve-like features from the image as described in the~\ref{subsec:ves} and~\ref{subsec:neurite}. Likewise, 3D phase congruency tensor can be performed using the tensor and then apply the Equations~\ref{eq:Vesselness} and~\ref{eq:Neuriteness}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%MORPHOLOGY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Enhancement with Mathematical Morphology}
\label{subsec:morph}
Another class of image enhancement method is based on mathematical morphology, is a technique for analysing the shapes and structures of the given data. 
Mathematical morphology has been used for several types of image processing or analyzing methods since it's been developed. Including image enhancement techniques, noise suppression, feature detection, and contrast sharpening or  pattern classification \cite{JWR2004}, enhancing depth-of-field \cite{DCC2006} and edge detection \cite{CWRTetal2002}. 

Mathematical morphology builds upon the idea of structural element which is describing the features with using the set of mathematical theory. In these methods mainly use combination of two operator which are non-linear in nature, and respectively dilation and erosion. These two operations take the image as an input and dilate or erode components within the particular area with structuring element.
Suppose that $I(\mathbf{p})$ is an image, and $S(\mathbf{p})$ is the structuring element for erosion $\ominus$ that describe the minimum of the points in the neighbourhood;
\begin{equation}
(I \ominus S)(\mathbf{p}) = \inf_{\mathbf{x} \in E}[I(\mathbf{x})+S(\mathbf{p}-\mathbf{x})],
\end{equation}
where $\inf$ the infimum and $\mathbf{x} \in E$ denotes all points in Euclidean space within the image. In the similar manner, dilation  $\oplus$ maximize points in the weighted neighbourhood described by the structuring element $S(\mathbf{p})$;
\begin{equation}
	(I \oplus S)(\mathbf{p}) = \sup_{\mathbf{x} \in E}[I(\mathbf{x})+S(\mathbf{p}-\mathbf{x})],
\end{equation}
where $\sup$ is the supremum. While erosion extends dark areas decreasing bright areas, dilation can expand bright areas and decrease dark areas. Using these tow operators, it can be defined four basic morphological filters which are:
\begin{align}
	\text{opening}: & \quad (I \circ S)(\mathbf{p}) = ((I \ominus S) \oplus S)(\mathbf{p})\\
	\text{closing}: & \quad (I \bullet S)(\mathbf{p}) = ((I \oplus S) \ominus S)(\mathbf{p})\\
	\text{top-hat}: & \quad TH(I(\mathbf{p})) = I(\mathbf{p}) - (I \circ S)(\mathbf{p})\\
	\text{bottom-hat}: & \quad BH(I(\mathbf{p})) = I(\mathbf{p}) - (I \bullet S)(\mathbf{p}).
\end{align}
The closing preserves bright structures while suppressing dark patterns meantime the opening maintains dark structures and patterns and suppressing bright features. Top-hat and bottom-hat transform enhance bright and dark regions, where those patterns correspond to the structuring element used.
\vspace{-15px}

==> tex/keyword.tex <==
\begin{keyword}
	3D image enhancement, 3D mathematical morphology, curvilinear features, bowler-hat transform
\end{keyword}
